Objaverse: A Universe of Annotated 3D Objects

Massive data corpora like WebText, Wikipedia, Conceptual Captions, WebImageText, and LAION have propelled recent dramatic progress in AI. Large neural models trained on such datasets produce impressive results and top many of today's benchmarks. A notable omission within this family of large-scale datasets is 3D data. Despite considerable interest and potential applications in 3D vision, datasets of high-fidelity 3D models continue to be mid-sized with limited diversity of object categories. Addressing this gap, we present Objaverse 1.0, a large dataset of objects with 800K+ (and growing) 3D models with descriptive captions, tags, and animations. Objaverse improves upon present day 3D repositories in terms of scale, number of categories, and in the visual diversity of instances within a category. We demonstrate the large potential of Objaverse via four diverse applications: training generative 3D models, improving tail category segmentation on the LVIS benchmark, training open-vocabulary object-navigation models for Embodied AI, and creating a new benchmark for robustness analysis of vision models. Objaverse can open new directions for research and enable new applications across the field of AI.

==> ali_intro.tex <==
Option 1:

1) our world is 3D
2) we have successfully approached some of the fundamental problems in computer vision in 2D projections of the 3D world (cameras, etc). 
3) Another, often disjoint, set of problems have also been conventionally studies in 3D (reconstruction, etc). 
4) The 2D side has seen amazing progress partly due to the availability of large scale rich 2D datasets.
5) it is much easier to  capture in 2d, scalable, large scale, web etc
6) The 3D side is on the verge of the same explosion. The main blocker is a large scale 3D data. 
7) We introduce objaverse 


Option 2:
1) Classical problems in vision is divided in disjoint categories of 2D and 3D. There is very little cross talk. 
2)  Our world is 3D, some problems are better suited to be explored in 2D, some in 3D and some jointly with intertwined solution across both. 
3) BEst known solutions in 2D are there because we have large scale data in 2D. 
4) The approach in 3D has been historically different with focus on smaller groups etc. Even NERF etc are mainly focused on a single scene etc. 
4) We argue that the cross talk is not there because of the lack of large scale data in 3D. 
5) If such a data exists research can study problems where it is most natural to be explored. 
6( We introduce objaverse blah
7) We picked problems across both 2D and 3D and show blahg.
8) A lot more can be done with this hybrid world1


3D -- mismatch in scale
mismatch in multi-modality

